Robust Online Video Instance Segmentation with Track Queries

Recently, transformer-based methods have achieved impressive results on Video Instance Segmentation (VIS). However, most of these top-performing methods run in an offline manner by processing the entire video clip at once to predict instance mask volumes. This makes them incapable of handling the long videos that appear in challenging new video instance segmentation datasets like UVO and OVIS. We propose a fully online transformer-based video instance segmentation model that performs comparably to top offline methods on the YouTube-VIS 2019 benchmark and considerably outperforms them on UVO and OVIS. This method, called Robust Online Video Segmentation (ROVIS), augments the Mask2Former image instance segmentation model with track queries, a lightweight mechanism for carrying track information from frame to frame, originally introduced by the TrackFormer method for multi-object tracking. We show that, when combined with a strong enough image segmentation architecture, track queries can exhibit impressive accuracy while not being constrained to short videos.

==> query_study.tex <==



\begin{figure*}[t]
  \centering
   \includegraphics[width=0.9\linewidth]{visualization/per_class_freq.pdf}
   \caption{\textbf{Instance class frequency of static queries on YouTube-VIS.} Evaluated on \texttt{val} split and plotted on log scale. \zitong{Labels on horizontal axis are grouped according to semantic similarity. }
%   Best viewed in color.
   } 
   \label{fig:per-class-freq}
\end{figure*}





\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=.95\linewidth]{visualization/position_legend.pdf}

   \caption{\textbf{Visualization of query firing patterns on UVO.} 
   Each dot is placed according to the instance's center of mass of the mask fired by the corresponding query, and darker dots imply larger object mask size. All images are normalized to dimension $480\times800$ before plotting firing patterns.
   Visualization includes the first 14 non-empty queries from the 50-query ResNet50 model on UVO \texttt{dense-val} split. 
%   Legend represents size of the mask using pixel as unit. 
   }
   \label{fig:uvo-firing-patterns}
\end{figure*}


\begin{figure}[t]
  \centering
   \includegraphics[width=.95\linewidth]{visualization/query_counts.pdf}

   \caption{\textbf{Object firing counts for static queries.} Results are generated for model with 100 static queries. YouTube-VIS result is evaluated on \texttt{val} split. UVO result is evaluated on \texttt{dense val} split. }
   \label{fig:count-stat}
\end{figure}
\subsection{\zitong{Detailed Study of Queries}} \label{sec:ablations}
Since UVO has the largest validation set among the three datasets, we perform our ablation study using UVO \texttt{dense-train} for training and \texttt{dense-val} for evaluation. 

% While static queries are an important component of 

% \input{tables/ablations}

\vspace{0.5em}
\noindent\textbf{Static query initialization}. 
% For the model parameter initialization happens before training, changing the number of static queries will cause such parameter's pretrained weights unusable. 
%  As a result, in all of our experiments we use randomly initialized queries.
We cannot change the number of static queries in a pretrained model without rendering the previously learned embedding representations unusable. As a result, we are curious about how important the image pretraining is for queries. We performed the following experiments on UVO using ResNet 50 backbone and MS COCO \cite{lin2014microsoft} pretrained model with 100 queries. On YouTube-VIS 2019, switching from pretrained queries to random initialized queries caused a 1 percent mAP decrease. In contrast, on the UVO dataset, we observed a 1 percent mAP \textit{increase}. This can be attributed to the following:
For the YouTubeVIS dataset, instance classes are a subset of MS COCO object classes. Thus, pretrained queries do a better job in firing on objects with similar semantics to the pretraining dataset. 
For the ``open world" UVO dataset, most objects belong to non-COCO categories. This means an MS COCO pretrained set of queries does not align well with the semantics of objects in UVO which have more diverse appearance compared with YouTube-VIS.



\vspace{0.5em}
\noindent\textbf{Number of static queries}. An increased number of queries typically allows the detector to capture more diverse object appearances. We performed the same study on the UVO dataset. In this study, all static query parameters are initialized as random values for fair comparison. To compensate for the effect of such an initialization, we increase learning rate for the query embeddings to be 4 times the global learning rate. 
We observe that performance peaks at 200 static queries, resulting in a 0.8 mAP accuracy increase compared with the 100 static query baseline. 
Counter to intuition, more queries (300 or more) are not helpful. This is due to the fact that the tracking-by-attention scheme only relies on static queries to predict the initial appearance of an object. Most object appearances are detected by track queries, and there are at most 1-2 new objects appearing in the middle of a video. Increasing the number of static queries also means each query is less likely to be assigned to a ground truth instance in $x^1$ during training. This may harm the quality of learned embeddings when training on smaller datasets like YouTube-VIS with few tracks annotated per video. Meanwhile, decreasing the query number by half does not harm performance. Furthermore, since computational cost scales quadratically w.r.t. the number of static queries, the 50 query experiment can be completed in only 100 minutes on 4 NVIDIA A40 GPUs. 
% \begin{figure}[t]
%   \centering
%   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    \includegraphics[width=0.8\linewidth]{figure/diagram-num-queries.pdf}

%    \caption{Trying different number of queries on UVO \texttt{dense-train} split. Evaluate on UVO \texttt{dense-val}}
%    \label{fig:uvo-num-queries}
% \end{figure}


% \begin{figure}[t]
%   \centering
%   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    \includegraphics[width=0.8\linewidth]{figure/diagram-frame-range.pdf}

%    \caption{Trying different frame range on UVO \texttt{dense-train} split. Evaluate on UVO \texttt{dense-val}}
%    \label{fig:uvo-frame-range}
% \end{figure}





% Ablation Study and 

To study the utilization of the static queries, we study its behavior compare trends on YouTube-VIS 2019 and UVO.

% using the 100-query model.

% trained and evaluated on the .


\vspace{0.5em}
\noindent\textbf{Query activity.} For YouTube-VIS, we found that there is usually one query that is significantly more active than other queries, as shown in Figure~\ref{fig:count-stat} (left). This is due to the fact that each frame in \ytbvis typically only contains a few objects centered in the frame. In contrast, UVO scenes are more crowded and show a more active query distribution in Figure~\ref{fig:count-stat} (right).
% and Figure~\ref{fig:count-stat-uvo50}. 
Furthermore, since YouTube-VIS contains class labels, we can also examine which class category instances belong to, as shown in Figure~\ref{fig:per-class-freq}.
This shows \zitong{objects with similar semantic meaning will likely be detected by the same} static queries. 




% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.0\linewidth]{visualization/count_stat_uvo100.pdf}

%   \caption{Bar plot of object firing count for static queries. Evaluated on UVO \texttt{dense val} split with model with 100 static queries.}
%   \label{fig:count-stat-uvo100}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.0\linewidth]{visualization/count_stat_uvo50.pdf}
%   \caption{Barplot of object firing count for static queries. Evaluated on UVO \texttt{dense val} split with model with 50 static queries.}
%   \label{fig:count-stat-uvo50}
% \end{figure}


\vspace{0.5em}
\noindent\textbf{Position study.} In addition to firing count, we are also interested in any trends in position and size of objects detected by static queries.
% We want to study the behavior of static queries in this section.
While the few very dominant queries in YouTube-VIS did not reveal very distinct trends, we found that UVO queries often specialize in particular regions or object sizes as shown in Figure~\ref{fig:uvo-firing-patterns}. Check supplementary material for visualization of other queries. 

% We used the validation set of YouTube-VIS to generate heatmaps, where brightness in the heatmap represents the number of masks a query fires at a specific position establishing a new track. Full brightness means the query always has an object fired at the location when there is a new object appearing in the frame. We show the corresponding heatmap of the most active query (the tallest red line in Figure~\ref{fig:count-stat}) in Figure~\ref{fig:ytvis-heatmap-1}. 






==> tables/ablations.tex <==
\begin{table} % [h]
    \centering
        \begin{subtable}{0.225\textwidth} % [h]
        \centering
        \begin{tabular}{c | c}
        \toprule
        \# of queries & AP \\
        \midrule
        50 & 21.0 \\
        100 & 21.1 \\
        200 & \textbf{21.8 }\\
        300 & 19.1 \\
        \bottomrule
        \end{tabular}
        \caption{Number of static queries}
        \label{tab:ablations_sq}
     \end{subtable}
     \hfill
    \begin{subtable}{0.225\textwidth} % [h]
        \centering
        \begin{tabular}{c | c}
        \toprule
        \# of frames & AP \\
        \midrule
        5 & 20.2 \\
        10 & 20.6 \\
        15 & \textbf{21.2} \\
        20 & 18.6 \\
        \bottomrule
       \end{tabular}
      \caption{Frame sampling range}
       \label{tab:ablations_fs}
    \end{subtable}
    % \vspace{-.5em}
     \caption{Evaluation on UVO \texttt{dense-val} split for different frame ranges and number of static queries in the model. A frame range of $n$ indicates that the frame $x_1$ is randomly sampled from the $n$ frames after or $n$ frames before $x_0$. All models were trained on the  UVO \texttt{dense-train} split.}
     \label{tab:ablations}
\end{table}
